Exact Simulation of Variance Gamma related OU processes: Application to the Pricing of Energy Derivatives

In this study we define a three-step procedure to relate the self-decomposability of the stationary law of a generalized Ornstein-Uhlenbeck process to the law of the increments of such processes. Based on this procedure and the results of Qu et al. (2019), we derive the exact simulation, without numerical inversion, of the skeleton of a Variance Gamma, and of a symmetric Variance Gamma driven Ornstein-Uhlenbeck process. Extensive numerical experiments are reported to demonstrate the accuracy and efficiency of our algorithms. These results are instrumental to simulate the spot price dynamics in energy markets and to price Asian options and gas storages by Monte Carlo simulations in a framework similar to the one discussed in Cummins et al. (2017, 2018).

==> Tables/TableGasStorageSpec.tex <==
\begin{table}
    \centering
    \begin{tabular}{|c|c|c|c|c|}
            \hline
             $C(0) $   &  $C(T) $ & $a_{in} $  & $a_{w}$ & $C_{max} $ \\
          \hline
             0  &  0 &  $1$ &  $1$ &  $20$ \\	
	    \hline
    \end{tabular}
    \small
    \caption{Fast Storage Specification.}\label{tab:storage:spec}
\end{table}

